Disentangling Causal Substructures for Interpretable and Generalizable Drug Synergy Prediction

Drug synergy prediction is a critical task in the development of effective combination therapies for complex diseases, including cancer. Although existing methods have shown promising results, they often operate as black-box predictors that rely predominantly on statistical correlations between drug characteristics and results. To address this limitation, we propose CausalDDS, a novel framework that disentangles drug molecules into causal and spurious substructures, utilizing the causal substructure representations for predicting drug synergy. By focusing on causal sub-structures, CausalDDS effectively mitigates the impact of redundant features introduced by spurious substructures, enhancing the accuracy and interpretability of the model. In addition, CausalDDS employs a conditional intervention mechanism, where interventions are conditioned on paired molecular structures, and introduces a novel optimization objective guided by the principles of sufficiency and independence. Extensive experiments demonstrate that our method outperforms baseline models, particularly in cold start and out-of-distribution settings. Besides, CausalDDS effectively identifies key substructures underlying drug synergy, providing clear insights into how drug combinations work at the molecular level. These results underscore the potential of CausalDDS as a practical tool for predicting drug synergy and facilitating drug discovery.

==> 6_Conclusions.tex <==
\section{Conclusions}
We have introduced a simple yet efficient loss function for pose estimation, based on the Wasserstein distance. Its ground metric represents the class correlation and can be predefined using an increasing function of arc length or learned by alternative optimization. Both the outlier and inlier noise in pose data are incorporated in a unimodal-uniform mixture distribution to construct the conservative label. We systematically discussed the fast closed-form solutions in one-hot and conservative label cases. The results show that the best performance can be achieved by choosing convex function, Binomial distribution for smoothing and solving its exact solution. Although it was originally developed for pose estimation, it is essentially applicable to other problems with discrete and periodic labels. In the future, we plan to develop a more stable adaptive ground metric learning scheme for more classes, and adjust the shape of conservative target distribution automatically.



\section{Acknowledgement}
The funding support from Youth Innovation Promotion Association, CAS (2017264), Innovative Foundation of
CIOMP, CAS (Y586320150) and Hong Kong Government General Research Fund GRF (Ref. No.152202/14E) are greatly appreciated.


